Dissecting strong-field excitation dynamics with atomic-momentum spectroscopy

Observation of internal quantum dynamics relies on correlations between the system being observed and the measurement apparatus. We propose using the center-of-mass (c.m.) degrees of freedom of atoms and molecules as a "built-in" monitoring device for observing their internal dynamics in non-perturbative laser fields. We illustrate the idea on the simplest model system - the hydrogen atom in an intense, tightly-focused infrared laser beam. To this end, we develop a numerically-tractable, quantum-mechanical treatment of correlations between internal and c.m. dynamics. We show that the transverse momentum records the time excited states experience the field, allowing femtosecond reconstruction of the strong-field excitation process. The ground state becomes weak-field seeking, an unambiguous and long sought-for signature of the Kramers-Henneberger regime.

==> xx-main.tex <==



==> xx-support.tex <==


